An LES study of turbulent flow over in-line tube-banks and comparison with experimental measurements

Turbulent flow across an in-line array of tube-banks with transverse and longitudinal pitch PT /D = 2.67, and PL /D = 2.31, has been simulated successfully by Large Eddy Simulation (LES) based on the dynamic Smagorinsky subgrid scale model (SGS), in which a wall-layer model is used to reduce the computational cost. The flow structures across the tube-banks were examined through the normalized Q criterion. The surface pressure characteristics from the middle cylinder within each column of cylinders are found to agree well with the existing experimental data, as did also the values of drag and lift coefficients. These results indicate that cylinders from the second column experience the minimum drag force and maximum lift force fluctuation. Spectral analyses were performed for velocity signals sampled behind each middle cylinder axis, which show that the dominant vortex shedding frequency does not vary across the tube-banks. On this basis, we also examined the shear layer instability. Finally, we report auto-correlation functions for streamwise and cross velocity fluctuations as a function of the spanwise length.

==> Makefile <==
# LaTeX Makefile
FILE=paper3_FTaC_2016_r0_arXiv

all: $(FILE).pdf

.PHONY: clean
clean:
	\rm *.aux *.blg *.out *.log
$(FILE).pdf: $(FILE).tex
	pdflatex $(FILE)
	bibtex $(FILE)
	pdflatex $(FILE)
	pdflatex $(FILE)

